Single Source - All Sinks Max Flows in Planar Digraphs

Let G = (V,E) be a planar n-vertex digraph. Consider the problem of computing max st-flow values in G from a fixed source s to all sinks t in V\{s}. We show how to solve this problem in near-linear O(n log^3 n) time. Previously, no better solution was known than running a single-source single-sink max flow algorithm n-1 times, giving a total time bound of O(n^2 log n) with the algorithm of Borradaile and Klein. An important implication is that all-pairs max st-flow values in G can be computed in near-quadratic time. This is close to optimal as the output size is Theta(n^2). We give a quadratic lower bound on the number of distinct max flow values and an Omega(n^3) lower bound for the total size of all min cut-sets. This distinguishes the problem from the undirected case where the number of distinct max flow values is O(n). Previous to our result, no algorithm which could solve the all-pairs max flow values problem faster than the time of Theta(n^2) max-flow computations for every planar digraph was known. This result is accompanied with a data structure that reports min cut-sets. For fixed s and all t, after O(n^{3/2} log^{3/2} n) preprocessing time, it can report the set of arcs C crossing a min st-cut in time roughly proportional to the size of C.

==> concluding.tex <==
We gave an $O(n\log^3n)$ time algorithm for the problem of finding max $st$-flow values for a fixed
source $s$ and all sinks $t\in V\setminus\{s\}$ in an $n$-vertex planar digraph $G = (V,E)$. The
previous best known solution was to perform $n - 1$ executions of a single-source single-sink max flow
algorithm, which gave an $O(n^2\log n)$ time bound with the algorithm of Borradaile and Klein~\cite{borradaile-09}.

An immediate corollary of our result is a near-quadratic time algorithm for finding max $st$-flow values for all
source/sink pairs $(s,t)$. We showed that the number of distinct max $st$-flow values is quadratic in
the worst case. Hence, our algorithm is optimal up to logarithmic factors.

Prior to this result, computing all max-flow values in a directed planar graph required up to $\Theta(n^2)$
max-flow computations.
We conjecture that a similar improvement is possible for general directed graphs. Another
interesting direction to pursue is to prove or disprove the existence of a data structure similar to the
oracle in~\cite{Borradaile2010}, which can answer queries for max $st$-flow values in constant time
after $o(n^2)$ preprocessing. A related question is whether it is possible to improve the time needed to find max $st$-flow values for
$k$ given input pairs $(s,t)$? Also, is it possible to remove the log-factors, i.e., compute all max-flow values in optimal $O(n^2)$ time?
Finally, our algorithm computes all cut-sets $\mathcal{C}$ in a planar digraph in $O(\min\{n^{5/2}\log^{3/2} n + \sum_{C\in \mathcal{C}} |C| \log \log n,n^{8/3}\log^{2/3} n + \sum_{C\in \mathcal{C}} |C|\})$ time.
Is it possible to improve this running time?
 


==> forest.tex <==
By assumption, $s$ is not a boundary vertex of any piece. For any outer boundary $C$ corresponding to a root in
$\mathcal F$, there is no other outer boundary in $\mathcal F$ separating $C$ and $s$.
Hence, every such $C$ must lie inside a hole in the same piece $P$.
Since $P$ has only $O(1)$ holes, the first part of the lemma follows.

For a node of $\mathcal F$ to be a child of another node in $\mathcal F$, the outer boundaries corresponding to these
nodes must share vertices with holes of the same piece. The second part of the lemma follows, again since a piece only has $O(1)$
holes and each piece is divided into a constant number of connected subpieces.
